General sum stochastic games with networked information flows

Inspired by applications such as supply chain management, epidemics, and social networks, we formulate a stochastic game model that addresses three key features common across these domains: 1) network-structured player interactions, 2) pair-wise mixed cooperation and competition among players, and 3) limited global information toward individual decision-making. In combination, these features pose significant challenges for black box approaches taken by deep learning-based multi-agent reinforcement learning (MARL) algorithms and deserve more detailed analysis. We formulate a networked stochastic game with pair-wise general sum objectives and asymmetrical information structure, and empirically explore the effects of information availability on the outcomes of different MARL paradigms such as individual learning and centralized learning decentralized execution.

==> ma_actor_critic.tex <==
\section{Actor Critic algorithms for finding Nash equilibria}
In problems listed in Section(CITE), we tend to be restricted to continuous state-action type algorithms. The reasn
Within a network stochastic game, players are biased towards withholding information from one another for many reasons. 
\subsection{Deep deterministic Policy Gradient}
DDPG is an actor-critic RL solution for single player MDPs that utilizes two function approximators to estimate the policy $\pi$ that  maximizes the player's expected reward. In this actor-critic approach, the \emph{policy} is approximated using neural networks as $\mu(\cdot; \theta_a)$, where the input is the information available to the actor, and $\theta_a$ are the parametrization variables for $\mu$. Similarly, the Q-value function is approximated as  $Q(\cdot, \cdot; \theta_c)$ and parametrized by $\theta_c$. The policy network is utilized to maximize the infinite horizon discounted reward for each player, 
\begin{equation}\label{eqn:actor_objective}
    J(\theta_a) = \max_{s\sim\rho, a \sim \mu(\cdot; \theta_a)}[\sum_{t=0}^\infty\gamma^tR_i(s_t(i), a_t(i), d_t(i))] = \max_{s\sim\rho, a \sim \mu(\cdot; \theta_a)}[Q(s, a; \phi)]
\end{equation}
The Q-value function network, also the critic, takes a one-step state-action-reward sequence given by $(s,a)$, and predicts its optimal value $Q(s,a)$. The objective of the Q-value function network is to minimize the least squares loss of $Q(\cdot, \cdot; \theta_c)$ given by 
\begin{equation}\label{eqn:critic_objective}
    L(\theta_c) = \mathbb{E}_{s, a, r, s^+ \sim \mc{D}}[Q(s,a;\theta_c) - (R(s,a) + \gamma \max_{a'}Q'(s', a'; \theta_c)]
\end{equation}
The critic network then is used to \emph{approximate} the gradient of the actor network by using the chain rule on~\eqref{eqn:actor_objective} as follows:
\begin{multline}\label{eqn:gradient_ddpg}
    \nabla_{\theta_a} J(\theta_a) \approxeq \mathbf{s \sim \mc{D}}[\nabla_\theta Q(s, \mu(s; \theta_a); \theta_c)]= \mathbf{E}_{s\sim\mc{D}}[\nabla_\theta \mu_{\theta}(s; \theta_a) \nabla_a Q(s, \mu(s; \theta_a); \theta_c)]
\end{multline}
Using~\eqref{eqn:gradient_ddpg}, DDPG iteratively updates the actor and critic networks to converge to the optimal policy $\mu(s; \theta_a^\star)$, $\forall s \in \mc{S}$. 
\subsection{Information access}

